Can the accuracy bias by facial hairstyle be reduced through balancing the training data?

Appearance of a face can be greatly altered by growing a beard and mustache. The facial hairstyles in a pair of images can cause marked changes to the impostor distribution and the genuine distribution. Also, different distributions of facial hairstyle across demographics could cause a false impression of relative accuracy across demographics. We first show that, even though larger training sets boost the recognition accuracy on all facial hairstyles, accuracy variations caused by facial hairstyles persist regardless of the size of the training set. Then, we analyze the impact of having different fractions of the training data represent facial hairstyles. We created balanced training sets using a set of identities available in Webface42M that both have clean-shaven and facial hair images. We find that, even when a face recognition model is trained with a balanced clean-shaven / facial hair training set, accuracy variation on the test data does not diminish. Next, data augmentation is employed to further investigate the effect of facial hair distribution in training data by manipulating facial hair pixels with the help of facial landmark points and a facial hair segmentation model. Our results show facial hair causes an accuracy gap between clean-shaven and facial hair images, and this impact can be significantly different between African-Americans and Caucasians.

==> table_exp1.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{c|ccc|ccc}
\multirow{1}{*}{Train} & \multicolumn{6}{c}{Test} \\
\cline{2-7}
& \multicolumn{3}{c|}{AAM} & \multicolumn{3}{c}{CM} \\
\cline{2-7}
& CS-CS & CS-FH & FH-FH & CS-CS & CS-FH & FH-FH \\
\cline{1-7}
0 CS 5000 FH & $5.12\pm0.07$ & $5.19\pm0.05$ & $5.91\pm0.04$ & $5.16\pm0.03$ & $4.52\pm0.04$ & $5.50\pm0.06$ \\
\cline{1-7}
500 CS 4500 FH & $5.16\pm0.06$ & $5.17\pm0.04$ & $5.91\pm0.04$ & $5.19\pm0.04$ & $4.47\pm0.07$ & $5.50\pm0.06$ \\
\cline{1-7}
1000 CS 4000 FH & $5.17\pm0.03$ & $5.19\pm0.05$ & $5.90\pm0.05$ & $5.20\pm0.03$ & $4.46\pm0.07$ & $5.52\pm0.06$ \\
\cline{1-7}
1500 CS 3500 FH & $5.21\pm0.04$ & $5.21\pm0.05$ & $5.89\pm0.05$ & $5.24\pm0.04$ & $4.50\pm0.09$ & $5.54\pm0.06$ \\
\cline{1-7}
2000 CS 3000 FH & $5.16\pm0.03$ & $5.19\pm0.03$ & $5.88\pm0.02$ & $5.26\pm0.02$ & $4.56\pm0.07$ & $5.57\pm0.07$ \\
\cline{1-7}
2500 CS 2500 FH & $5.17\pm0.07$ & $5.19\pm0.03$ & $5.83\pm0.03$ & $5.30\pm0.05$ & $4.62\pm0.05$ & $5.54\pm0.04$ \\
\cline{1-7}
3000 CS 2000 FH & $5.19\pm0.08$ & $5.21\pm0.05$ & $5.83\pm0.05$ & $5.31\pm0.04$ & $4.59\pm0.03$ & $5.58\pm0.05$ \\
\cline{1-7}
3500 CS 1500 FH & $5.20\pm0.05$ & $5.26\pm0.06$ & $5.80\pm0.04$ & $5.30\pm0.03$ & $4.60\pm0.05$ & $5.52\pm0.07$ \\
\cline{1-7}
4000 CS 1000 FH & $5.23\pm0.08$ & $5.31\pm0.01$ & $5.81\pm0.04$ & $5.34\pm0.03$ & $4.65\pm0.04$ & $5.47\pm0.12$ \\
\cline{1-7}
4500 CS 500 FH & $5.16\pm0.04$ & $5.28\pm0.04$ & $5.71\pm0.04$ & $5.37\pm0.02$ & $4.71\pm0.02$ & $5.45\pm0.08$ \\
\cline{1-7}
5000 CS 0 FH & $5.17\pm0.08$ & $5.29\pm0.06$ & $5.75\pm0.07$ & $5.35\pm0.01$ & $4.76\pm0.04$ & $5.36\pm0.04$ \\
\cline{1-7}

\end{tabular}
\caption{D-prime values between genuine and impostor distributions for African-American (AAM) and Caucasian (CM) males. The same number of clean-shaven (CS) and facial hair (FH) images are selected for each subjects to create 13 training sets.}
\label{tab:dprime_exp1}
\end{table*}

